DisCoF$^+$: Asynchronous DisCoF with Flexible Decoupling for Cooperative Pathfinding in Distributed Systems

In our prior work, we outlined an approach, named DisCoF, for cooperative pathfinding in distributed systems with limited sensing and communication range. Contrasting to prior works on cooperative pathfinding with completeness guarantees, which often assume the access to global information, DisCoF does not make this assumption. The implication is that at any given time in DisCoF, the robots may not all be aware of each other, which is often the case in distributed systems. As a result, DisCoF represents an inherently online approach since coordination can only be realized in an opportunistic manner between robots that are within each other's sensing and communication range. However, there are a few assumptions made in DisCoF to facilitate a formal analysis, which must be removed to work with distributed multi-robot platforms. In this paper, we present DisCoF$^+$, which extends DisCoF by enabling an asynchronous solution, as well as providing flexible decoupling between robots for performance improvement. We also extend the formal results of DisCoF to DisCoF$^+$. Furthermore, we evaluate our implementation of DisCoF$^+$ and demonstrate a simulation of it running in a distributed multi-robot environment. Finally, we compare DisCoF$^+$ with DisCoF in terms of plan quality and planning performance.

==> sections/problem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{PRELIMINARIES}


First, we formulate the multi-robot coordination problem with conflicts. 
We assume the existence of a team of $N$ robots $R = \{r_i\}_{i \in \{1..N\}}$.
All the robots operate within the same workspace $\Wc$. 
The workspace is abstracted into a finite representation through a graph $G = (V,E)$ using a cell decomposition method, 
or a roadmap method etc. \cite{LaValle05}
Here, $V$ is a set of vertices where each vertex $v$ represents a cell in the decomposition or a waypoint on the roadmap 
and $E$ is a set of edges connecting the vertices.
For simplicity in the presentation, we will assume that all robots share the same abstraction of the environment.


The motion of each robot in the workspace is modeled as a labeled Finite State Machine (FSM).
Thus, we assume a unique Finite Transition System (FTS) $\FTS_i$ for each robot $i$.


Each state of the FTS $\FTS$ is labeled by a number of symbols (i.e., propositions) from a set $\Pi= \{\pi_0,$ $\pi_1,$ $\dots,$ $\pi_n\}$ 
that represent regions in the state space of the robot or, more generally, actions that can be performed by the robot.


\begin{defn} [FTS] A Finite Transition System is a tuple $\FTS = (Q, q_0, \rightarrow_\FTS, L, F)$ where:
$Q \subseteq V$ is a set of states; 
$q_0 \in Q$ is the initial state; 
$\rightarrow_\FTS$  is the transition relation;  
$L : Q \rightarrow \Pc(\Pi)$ maps each state $q$ to the set of atomic propositions that are true on $q$; and,
$F \subseteq Q$ is a set of goal states.
\end{defn}


We define a {\it path} $p : \Ne \rightarrow Q$ on the FSM to be a sequence of states and a {\it trace} to be the corresponding sequence of sets of propositions.
Formally, a path is a function $p : \Ne \rightarrow Q$ such that for each $i\in \Ne$ we have $p(i) \rightarrow_\FTS p(i+1)$ and the trace is the function composition $\bar p = L \circ p : \Ne \rightarrow \Pc(\Pi)$.
The language $\Lc(\FTS)$ of $\FTS$ consists of all possible traces.

The concurrent operation of all the robots within the workspace is modeled through the synchronous composition of the FSM representing each robot.

\begin{defn} [Synchronous Composition] 
Given two FTS $\FTS_1$ and $\FTS_2$, the synchronous composition $\FTS_1 \times \FTS_2$ is a new FTS $\FTS = (Q, q_0, \rightarrow_\FTS, L, F)$ where:
$Q = Q_1 \times Q_2$; 
$q_0  = (q_{01}, q_{02})$; 
$q = (q_1,q_2) \rightarrow_\FTS q' = (q_1',q_2')$  iff $q_1 \rightarrow_{\FTS_1} q'_1$ and $q_2 \rightarrow_{\FTS_2} q'_2$;  
$L : Q \rightarrow \Pc(\Pi)^2$ with $L(q_1,q_2) = (L(q_1),L(q_2))$; and,
$F = F_1\times F_2$.
\end{defn}
%\todo[inline]{note that $\rightarrow_{\FTS_1}$ and $\rightarrow_{\FTS_2}$ are different}
%\todo[inline]{no need for the $q_2' \neq q_2$ above, so removed}

Given an FTS $\FTS$ that models the concurrent operation of $N$ robots, our goal is to find a plan that will navigate the robots from their initial states $q_0$ to some goal states in $F$.
%Extending the goal to include LTL formulas is to be considered in future work.

\begin{defn} [Plan] 
A plan on an FTS $\FTS = (Q, q_0, \rightarrow_\FTS, L, F)$ is a finite path $p$ such that $p(0) = q_0$ and there exists some $n \in \Ne$ such that $p(n) \in F$. 
There is also a cost associated with $p$.
\end{defn}

\begin{defn} [Plan Restrictions] 
Plan restrictions are the set of predefined (temporal) constraints on $V$ that must be satisfied by the plan on the FTS of the robots. 
\end{defn}

For example, a plan restriction may require that $q_{ti} \cap q_{tj} (i \neq j) \equiv \emptyset$, which means that the same element in $V$ cannot appear simultaneously in the states of two different robots. 
%More complex plan restrictions can also be implemented as Buchi Automata [cite].
%\todo[inline]{TONY: is this right?}

\begin{defn} [Conflicts] 
Conflicts are violations of plan restrictions on $V$.
\end{defn}

We denote that there is a {\em conflict relation} for $R_1 \subseteq R$ in the next $h$ steps as $\diamond_h R_1$, such that there exists a conflict when all the robots in $R_1$ follow their current plans in the next $h$ steps while ignoring the influence from the other robots; furthermore, we require that $\diamond_h$ be minimal, such that any $R_2 \subset R_1$ does not introduce the same conflict. 
%Furthermore, we define a transitive conflicting relation, denoted by $\Delta_h$, such that $r \Delta_h r''$ if: $1)$ $r \Delta_h r'$ and $r' \Delta r''$, or $2)$ $r \diamond r''$.

\begin{prob}
Given a team of $N$ robots, compute a plan $p$ without conflicts. 
\end{prob}

%\todo[inline]{Reiterate on contributions}

%Extending the goal to include LTL formulas is to be considered in future work.

